Inferring Latent Market Forces: Evaluating LLM Detection of Gamma Exposure Patterns via Obfuscation Testing

We introduce obfuscation testing, a novel methodology for validating whether large language models detect structural market patterns through causal reasoning rather than temporal association. Testing three dealer hedging constraint patterns (gamma positioning, stock pinning, 0DTE hedging) on 242 trading days (95.6% coverage) of S&P 500 options data, we find LLMs achieve 71.5% detection rate using unbiased prompts that provide only raw gamma exposure values without regime labels or temporal context. The WHO-WHOM-WHAT causal framework forces models to identify the economic actors (dealers), affected parties (directional traders), and structural mechanisms (forced hedging) underlying observed market dynamics. Critically, detection accuracy (91.2%) remains stable even as economic profitability varies quarterly, demonstrating that models identify structural constraints rather than profitable patterns. When prompted with regime labels, detection increases to 100%, but the 71.5% unbiased rate validates genuine pattern recognition. Our findings suggest LLMs possess emergent capabilities for detecting complex financial mechanisms through pure structural reasoning, with implications for systematic strategy development, risk management, and our understanding of how transformer architectures process financial market dynamics.

==> 00_Header.tex <==
\RequirePackage{silence}
\WarningFilter{latex}{Command \showhyphens has changed}

\IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{booktabs} % for professional tables
\usepackage{multirow}
\usepackage{url}
\usepackage[utf8]{inputenc}  % UTF-8 encoding support
\usepackage[T1]{fontenc}
\usepackage{gensymb} % Degree symbol and others
% For fixing specific issues:
\usepackage{lmodern} % Latin Modern fonts (better rendering)
\usepackage{microtype} % Better typography

% Hyperref configuration for IEEE Xplore compatibility
\usepackage[
    pdftex,
    pdfversion=1.5,           % IEEE requires PDF 1.5 or lower
    pdfa=true,                % PDF/A compliance (archival format)
    pdfstartview=FitH,        % Fit to width when opened
    pdfpagelayout=OneColumn,  % Single column view
    bookmarks=true,
    bookmarksopen=false,
    colorlinks=false,         % No colored links (IEEE standard)
    pdfborder={0 0 0},        % No link borders
    unicode=true              % Support Unicode characters
]{hyperref}

% PDF metadata (update with your information)
\hypersetup{
    pdftitle={Testing LLM Structural Reasoning in Market Microstructure Through Unbiased Obfuscation},
    pdfauthor={[Your Name]},
    pdfsubject={IEEE Big Data 2025},
    pdfkeywords={Large Language Models, Market Microstructure, Pattern Recognition, Obfuscation Testing, Gamma Exposure}
}

\usepackage{array}
\usepackage{adjustbox}
\usepackage{float}
% \usepackage[font=footnotesize,labelfont=bf]{caption}
% \captionsetup{compatibility=false}

\setlength{\tabcolsep}{5pt} % default is 6pt
% % Adjust header height to avoid fancyhdr warning
% \setlength{\headheight}{14.5pt}
% \addtolength{\topmargin}{-2.5pt}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
